4DLangVGGT: 4D Language-Visual Geometry Grounded Transformer

Constructing 4D language fields is crucial for embodied AI, augmented/virtual reality, and 4D scene understanding, as they provide enriched semantic representations of dynamic environments and enable open-vocabulary querying in complex scenarios. However, existing approaches to 4D semantic field construction primarily rely on scene-specific Gaussian splatting, which requires per-scene optimization, exhibits limited generalization, and is difficult to scale to real-world applications. To address these limitations, we propose 4DLangVGGT, the first Transformer-based feed-forward unified framework for 4D language grounding, that jointly integrates geometric perception and language alignment within a single architecture. 4DLangVGGT has two key components: the 4D Visual Geometry Transformer, StreamVGGT, which captures spatio-temporal geometric representations of dynamic scenes; and the Semantic Bridging Decoder (SBD), which projects geometry-aware features into a language-aligned semantic space, thereby enhancing semantic interpretability while preserving structural fidelity. Unlike prior methods that depend on costly per-scene optimization, 4DLangVGGT can be jointly trained across multiple dynamic scenes and directly applied during inference, achieving both deployment efficiency and strong generalization. This design significantly improves the practicality of large-scale deployment and establishes a new paradigm for open-vocabulary 4D scene understanding. Experiments on HyperNeRF and Neu3D datasets demonstrate that our approach not only generalizes effectively but also achieves state-of-the-art performance, achieving up to 2% gains under per-scene training and 1% improvements under multi-scene training. Our code released in https://github.com/hustvl/4DLangVGGT

==> src/method.tex <==
\section{Methodology: 4DLangVGGT}
% Our method, 4DLangVGGT, is a unified pipeline for constructing language-aware 4D fields. 
% We start by detailing feature extraction in Section 4.1, introduce the semantic bridging decoder for semantic alignment in Section 4.2, and conclude with the training loss in Section 4.3.

Our proposed framework, \textbf{4DLangVGGT}, introduces a unified approach to construct \emph{language-aware 4D fields} that is both geometrically faithful and semantically aligned. The method is designed around three main components: (i) a geometry-driven feature extraction stage powered by StreamVGGT, (ii) a \emph{Semantic Bridging Decoder} (SBD) that maps spatio-temporal geometry tokens into language-aligned embeddings, and (iii) a multi-objective training strategy that jointly optimizes semantic alignment and appearance reconstruction. An overview of the framework is provided in Figure~\ref{fig:fig2}.


% The pipeline consists of three main stages: (i) Feature Extraction, where a frozen StreamVGGT encoder that extracts geometry features from input videos, and (ii) Semantic Bridging Decoder(SBD), a semantic field construction module, which employs a DPT backbone followed by two task-specific heads. An overview of the architecture is shown in Figure\ref{fig:fig2}.

% Our goal is to construct a unified 4D language-aware field model that supports both video reconstruction and semantic prediction. 
% The proposed framework consists of two main components: 
% (i) a frozen StreamVGGT encoder that extracts spatio-temporal features from input videos, and 
% (ii) a semantic field construction module, which employs a DPT backbone followed by two task-specific heads. 

Formally, given input sequence $\{\mI_t\}_{t=1}^T$, our goal is to construct a 4D semantic field $f_{\mathrm{lang}}(\cdot)$ that supports open-vocabulary queries while maintaining geometric and temporal coherence. The pipeline proceeds in three steps:

\begin{enumerate}
    \item \textbf{StreamVGGT Encoder-Decoder.} Each frame $\mI_t$ is passed through a frozen StreamVGGT encoder and decoder, producing spatio-temporal geometry tokens $\mG_t \in \sR^{h \times w \times C}$.
    \item \textbf{Semantic Bridging.} Geometry tokens are refined and projected into a language-aligned space via the Semantic Bridging Decoder (SBD), yielding semantic features $\hat{\mS}_t \in \sR^{h' \times w' \times D}$.
    \item \textbf{Supervision.} The SBD simultaneously performs semantic prediction and auxiliary RGB reconstruction, with joint losses ensuring both semantic grounding and perceptual fidelity.
\end{enumerate}

This formulation can be summarized as
\begin{equation}
f_{\mathrm{lang}}(I_t) = g_{\mathrm{SBD}}\left( \mathcal{A}(\mI_t, \sM_{t-1}) \right),
\end{equation}
where $\mathcal{A}$ denotes the frozen StreamVGGT aggregator with memory $\sM_{t-1}$, and $g_{\mathrm{SBD}}$ represents the Semantic Bridging Decoder.


\begin{figure}[t]
    \centering
    % \vspace{-0.4em}
    \includegraphics[width=1.0\linewidth]{figure/figure2.pdf}
    % \vspace{-1.8em}
    \caption{Illustration of 4DLangVGGT pipeline.}	
    % \vspace{-1em}
    \label{fig:fig2}
\end{figure}

% Our goal is to build a unified 4D language-aware field model that uses pixel-level language guidance as well as segmentation masks from an MLLM, so that the system simultaneously reconstructs videos and aligns/predicts semantic features. The guidance output from the SAM masks $+$ MLLM semantic features, which enforces finer semantic alignment, and the RGB reconstruction preserves the visual and geometric fidelity. In what follows, we describe the architecture and loss functions. 

\subsection{Semantic Bridging with StreamVGGT Tokens}
\label{sec:SBD}
\paragraph{StreamVGGT Encoder-Decoder.}
The StreamVGGT aggregator alternates between \emph{spatial attention} and \emph{temporal causal attention}, producing geometry tokens $\mG_t$ that encode both fine-grained 3D structure and temporal dynamics:
\begin{equation}
\mG_t = f_\mathrm{StreamVGGT}(\mI_t, \sM_{t-1}), \quad \mF_t \in \sR^{h \times w \times C}.
\end{equation}
Where $f_\mathrm{StreamVGGT}(\cdot)$ is StreamVGGT encoder and decoder, these frozen features serve as a geometry-centric basis for semantic alignment.

\paragraph{Semantic Bridging Decoder (SBD).}
Raw geometry tokens, while structurally accurate, are agnostic to semantics. To bridge this gap, we design the Semantic Bridging Decoder, which operates in two steps:

\begin{itemize}
    \item \textbf{Refinement.} A Dense Prediction Transformer (DPT) refines $\mF_t$ into contextually enriched representations:
    \begin{equation}
    \mH_t = \mathrm{DPT}(\mG_t), \quad \mH_t \in \sR^{h' \times w' \times C'}.
    \end{equation}
    This refinement incorporates long-range spatial and temporal dependencies, enabling robust contextual reasoning.
    
    \item \textbf{Dual-head Decoding.} From $\mH_t$, we derive both language-aligned features and appearance reconstructions:
    \begin{equation}
    \hat{\mS}_t = g_{\mathrm{Lang}}^{\mathrm{UNet}}(\mH_t), \quad \hat{\mI}_t = \sigma\!\left(g_{\mathrm{RGB}}^{\mathrm{UNet}}(\mH_t)\right),
    \end{equation}
    where $g_{\mathrm{Lang}}$ maps features into a $D$-dimensional semantic space, and $g_{\mathrm{RGB}}$ reconstructs RGB frames for perceptual consistency. The dual-head design enforces mutual guidance: semantic embeddings preserve structural fidelity, while RGB reconstruction is regularized by semantic supervision.
\end{itemize}




% \subsection{Feature Extraction with StreamVGGT}
% \subsection{Feature Extraction}
% \label{sec4.2}
% A core requirement for open-vocabulary 4D querying is to anchor semantic fields on reliable geometric representations that maintain spatial precision and temporal coherence. Prior work like 4D LangSplat depends on per-scene Gaussian optimization, whose scene-specific nature hinders scalability and query accuracy. To address this, we adopt the \textbf{StreamVGGT aggregator module}, which includes both the image encoder and the spatio-temporal decoder as a frozen feedforward feature extractor.

% \paragraph{Spatio-temporal Feature Extractor}  
% We use a pre-trained, denoted frozen StreamVGGT aggregator module. This module alternates between spatial attention and temporal causal attention to encode image tokens of each frame into geometry tokens $F_{t}$ rich in both geometric and temporal information:
% \begin{equation}
% F_t = \mathcal{A}(I_t, M_{t-1}), \quad F_t \in \mathbb{R}^{h \times w \times C},
% \end{equation}  
% where $M_{t-1}$ is cached memory of recent frames (e.g., last $K$ frames), giving spatio-temporal, geometrically informed features. $\mathcal{A}$ represents the aggregator module, which incorporates multiple layers of Spatial Attention and Temporal Causal Attention.

% \paragraph{Semantic Bridging Decoder (SBD)}  

% \lmh{4D recon tokeni...}

% The Semantic Bridging Decoder (SBD) plays a central role in our framework by aligning geometry-centric features with language semantics. Its primary objective is to perform semantic alignment on the geometry tokens $F_t$, mapping the dynamic, scene-aware features into a language-aligned semantic space. This alignment is critical for the construction of a 4D language field, since raw geometric features, although effective in capturing spatial and temporal structure, remain agnostic to high-level semantics. By bridging geometry and language domains, the SBD ensures that the learned representation is simultaneously aware of the evolving scene structure and capable of supporting open-ended semantic queries.

% To achieve this, we first refine the geometry tokens using a Dense Prediction Transformer (DPT). Unlike direct feed-forward mapping, the DPT introduces contextual reasoning across spatial and temporal dimensions, enabling each feature location to incorporate long-range dependencies from both its geometric neighborhood and its dynamic evolution across time. This refinement produces enhanced feature maps:

% \begin{equation}
% H_t = \mathrm{DPT}(F_t), \quad H_t \in \mathbb{R}^{h' \times w' \times C'}.
% \end{equation}
% Here, $H_t$ captures a rich representation that integrates structural fidelity from geometry with contextual cues necessary for semantic interpretation.

% From the refined features $H_t$, we design two complementary prediction heads:

% \begin{itemize}

% \item RGB Reconstruction Head. The RGB head is defined as $g_{\rm RGB} : \mathbb{R}^{h'\times w'\times C'} \to \mathbb{R}^{H \times W \times 3}$, producing reconstructed frames $\hat I_t = g_{\rm RGB}(H_t)$. Although reconstructing RGB images is not the final goal of our framework, it serves as an essential auxiliary supervision signal. RGB signals contain dense appearance information such as textures, color distributions, and material boundaries, which are difficult to infer solely from geometric features. By encouraging the model to recover RGB appearance, the network is guided to preserve perceptually meaningful details in $H_t$, which in turn facilitates more accurate and discriminative semantic feature learning. Intuitively, reconstructing the video forces the model to “understand” the scene holistically, ensuring that the learned features are sensitive to subtle visual cues that might otherwise be overlooked. In practice, this auxiliary task significantly improves the stability and expressiveness of the semantic representations, even though the RGB head itself is discarded during inference.

% \item Language Feature Head. The language head is defined as $g_{\rm Lang} : \mathbb{R}^{h'\times w'\times C'} \to \mathbb{R}^{h'\times w'\times D}$, producing semantic features $\hat S_t = g_{\rm Lang}(H_t)$. These features are aligned with the language embedding space and form the basis of the constructed 4D language field. Unlike the RGB reconstruction task, which focuses on capturing appearance-level information, the language head directly projects $H_t$ into a high-dimensional semantic embedding, making the representation queryable by natural language. The semantic features $\hat S_t$ thus encapsulate both geometric grounding and linguistic interpretability, enabling downstream tasks such as open-vocabulary recognition, temporal reasoning, and interactive querying.

% \end{itemize}

% \paragraph{Semantic Bridging Decoder}
% Given the refined features $H_t \in \mathbb{R}^{h' \times w' \times C'}$, the Semantic Bridging Decoder employs two parallel decoding branches: a language-aligned semantic head and an auxiliary RGB reconstruction head. Formally, we define

% \begin{equation}
% \hat S_t = g_{\text{Lang}}(H_t), \quad
% \hat I_t = g_{\text{RGB}}(H_t),
% \end{equation}

% where $g_{\text{Lang}} : \mathbb{R}^{h' \times w' \times C'} \to \mathbb{R}^{h' \times w' \times D}$ denotes the semantic projection function, which maps the geometry and features that are aware of the environment to a $D$ dimensional embedding space aligned with language semantics. The output $\hat S_t$ thus encodes high-level concepts that can be directly associated with textual supervision.
% Meanwhile, $g_{\text{RGB}} : \mathbb{R}^{h' \times w' \times C'} \to \mathbb{R}^{H \times W \times 3}$ denotes the appearance reconstruction branch, which aims to reconstruct the original RGB frame $\hat I_t$ at the pixel level. This auxiliary reconstruction task provides low-level structural and perceptual guidance, ensuring that the learned features preserve fine-grained visual fidelity.

% To further enhance semantic grounding, the semantic head produces multi-scale feature embeddings:

% \begin{equation}
% \hat S_t = g_{\text{Lang}}(H_t),
% \end{equation}

% where different spatial resolutions are decoded to capture both global context (coarse-scale semantics) and local details (fine-scale attributes). This facilitates robust alignment with language descriptions at varying levels of granularity.

% In parallel, the RGB reconstruction head adopts a UNet-based decoder followed by a sigmoid activation:

% \begin{equation}
% \hat I_t = \sigma\left(g_{\text{RGB}}^{\text{UNet}}(H_t)\right), \quad \hat I_t \in [0,1]^{H \times W \times 3},
% \end{equation}

% where $\sigma(\cdot)$ normalizes the output to the valid image range. This design enforces perceptual consistency with the input video frames and prevents the semantic features from drifting away from appearance realism.

% Importantly, the dual-head design provides mutual guidance: the semantic projection benefits from the RGB reconstruction constraint, which preserves spatial and structural fidelity, while the RGB reconstruction is regularized by semantic supervision, encouraging it to capture not only appearance but also concept-level consistency. By training the two heads jointly, the model learns features that are simultaneously semantically discriminative and visually faithful, achieving a stronger 4D language-based representation.

% Formally, consider a video represented as a sequence of frames
% \[
% \mathcal{V} = \{I_t\}_{t=1}^T,\quad I_t\in\mathbb{R}^{H\times W\times3}.
% \]
% At each time step \(t\), the aggregator module produces:
% \begin{equation}
% F_t = \mathcal{A}(I_t, M_{t-1}),
% \end{equation}
% where \(F_t\in\mathbb{R}^{h\times w\times C}\) is the feature map at frame \(t\), and \(M_{t-1}\) denotes the cached memory of past key–value tokens. This mechanism enables temporal-aware feature extraction without future-frame leakage.

% To keep inference efficient over long video streams, we limit the memory to the most recent \(K=128\) frames:
% \begin{equation}
% M_{t} = \{F_{\max(1, t-K+1)}, \dots, F_{t}\}.
% \end{equation}
% This choice balances temporal context retention with bounded computation and GPU memory usage, mitigating overhead as video length increases.

% The StreamVGGT aggregator is based on a causal transformer architecture with temporal causal attention and memory caching. By utilizing the full aggregator (image encoder + spatio-temporal decoder), our pipeline inherits temporally consistent and high-quality geometric features suitable for open-vocabulary 4D querying. Importantly, since this module is shared across all scenes, it eliminates the need for per-scene retraining while providing a stable geometric foundation for downstream semantic field learning.
% \subsection{Semantic Field Construction}

% \paragraph{Architecture} 
% With temporally coherent geometric features \(\{F_t\}\) obtained from the StreamVGGT aggregator module, we design a semantic field construction pipeline that jointly supports language-grounded semantic prediction and high-fidelity RGB reconstruction while retaining a cohesive architecture.

% Each frame’s feature \(F_t \in \mathbb{R}^{h \times w \times C}\) is first passed through a Dense Prediction Transformer (DPT) to produce a refined representation:
% \begin{equation}
% H_t = \mathrm{DPT}(F_t), \quad H_t \in \mathbb{R}^{h' \times w' \times C'}.
% \end{equation}
% We employ DPT due to its global receptive field and context integration capabilities, which have been shown to significantly improve dense prediction tasks such as semantic segmentation and monocular depth estimation. The transformer’s ability to maintain high-resolution activations throughout its depth ensures that both local detail and global structure are preserved—crucial for accurately grounding semantics in a dynamic 4D setting.

% From \(H_t\), we derive two parallel outputs via dedicated lightweight heads: an RGB Head that reconstructs the input video frame,
% \[
% \hat{I}_t = g_{\mathrm{RGB}}(H_t),
% \]
% and a Language Head that predicts a dense semantic feature embedding,
% \[
% \hat{S}_t = g_{\mathrm{Lang}}(H_t).
% \]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% \paragraph{Training Loss}
% The RGB Head enforces visual fidelity by reconstructing \(I_t\), while the Language Head ensures that \(H_t\) encodes language-aligned semantics for open-vocabulary querying. We jointly optimize with a multi-task loss:
% \[
% \mathcal{L}_{\mathrm{RGB}} = \|\hat{I}_t - I_t\|_2^2,\quad
% \mathcal{L}_{\mathrm{Lang}} = \|\hat{S}_t - S_t\|_2^2,\quad
% \mathcal{L}_{\mathrm{total}} = \mathcal{L}_{\mathrm{RGB}} + \lambda\,\mathcal{L}_{\mathrm{Lang}},
% \]
% where \(S_t\) is the ground-truth semantic embedding (e.g., CLIP or MLLM output), and \(\lambda\) balances the two objectives.

% Integrating the dual-head design within the shared DPT backbone offers several benefits: the RGB supervision acts as an implicit regularizer, preventing overfitting to semantic embeddings and ensuring that geometric fidelity is maintained; the shared representation supports both tasks efficiently, avoiding parameter redundancy; and DPT’s global context integration ensures that the semantic predictions are spatially consistent and contextually grounded. Overall, this design enables accurate reconstruction and robust semantic grounding in a unified and scalable framework for open-vocabulary 4D querying.

% \subsection{Training Losses}

% \paragraph{Semantic Ground Truth} 
% For each frame \(f_{i_t}\) in Video $V_i = \{f_{i_1},f_{i_2},\cdots,f_{i_n}\}$, we also assume access to:
% \begin{itemize}

% \item  A segmentation map (mask) \(\mathrm{Seg}_t \in \{0,1, \cdots, m\}^{h \times w}\) produced by an SAM (where $m$ is the total object ids in a video), indicating which pixels correspond to a query or class of interest.  
% \item A dense semantic feature map \(\mathrm{S}_t \in \mathbb{R}^{h \times w \times D}\), for example, features from a CLIP vision encoder or other language-aligned model.

% \end{itemize}

% \paragraph{Semantic Alignment Loss.}
% We first restrict semantic supervision to the masked regions, ensuring alignment focuses on meaningful areas. Let 
% \begin{equation}
% \hat S_t^{(m)} = \mathrm{Seg}_t \odot \hat S_t, \qquad
% \mathrm{S}_t^{(m)} = \mathrm{Seg}_t \odot \mathrm{S}_t,
% \end{equation}
% where $\odot$ denotes element-wise multiplication.

% The alignment loss consists of an $L_1$ regression term for absolute closeness and a cosine similarity term for directional alignment in the embedding space:
% \begin{equation}
% \mathcal{L}_{\rm lang}^{(L_1)}(t) = \| \hat S_t^{(m)} - \mathrm{S}_t^{(m)} \|_1,
% \end{equation}
% \begin{equation}
% \mathcal{L}_{lang}^{(\cos)}(t) = 1 - \frac{ \langle \hat S_t^{(m)}, \mathrm{S}_t^{(m)} \rangle }{ \|\hat S_t^{(m)}\|_2 \|\mathrm{S}_t^{(m)}\|_2 }
% \end{equation}

% The final semantic alignment loss is
% \begin{equation}
% \mathcal{L}_{lang}(t) = \lambda_1 \mathcal{L}_{lang}^{(L_1)}(t) + \lambda_2 \mathcal{L}_{\rm lang}^{(\cos)}(t),
% \end{equation}
% where $\lambda_1$ and $\lambda_2$ control the balance between absolute alignment and angular consistency.

% \paragraph{Image Reconstruction Loss.}
% To maintain perceptual fidelity and stabilize semantic learning, the image reconstruction branch is supervised via a hybrid $L_1$–$L_2$ loss:
% \begin{equation}
% \mathcal{L}_{rec}(t) = \lambda_{img} \| \hat I_t - I_t \|_1 + (1 - \lambda_{img}) \|\hat I_t - I_t \|_2^2,
% \end{equation}
% where $\lambda{\rm img} \in [0,1]$ interpolates between the accuracy of the pixel-level ($L_1$) and smoother reconstruction ($L_2$).

% \paragraph{Joint Training Objective.}
% The final training loss jointly optimizes both semantic grounding and visual reconstruction:
% \begin{equation}
% \mathcal{L} = \alpha \sum_t \mathcal{L}_{lang}(t) + \beta \sum_t \mathcal{L}_{rec}(t),
% \end{equation}
% where $\alpha$ and $\beta$ balance the contributions of the two objectives.


% This dual-head supervision provides mutual benefits:

% \begin{itemize}
% \item The semantic loss ensures that the features $\hat S_t$ are aligned with language semantics, pushing the representation toward conceptually meaningful directions.

% \item The loss of image reconstruction anchors the features to spatial and perceptual fidelity, preventing semantic embeddings from drifting away from the underlying visual content.

% \item By training jointly, the semantic branch benefits from stable low-level cues preserved by RGB reconstruction, while the reconstruction branch is implicitly regularized by semantic alignment, encouraging reconstructions that are not only visually realistic, but also semantically consistent.

% \item As a result, the model learns a representation space that is visually faithful and semantically aligned simultaneously, which is crucial for 4D language-based video understanding and generation.
% \end{itemize}

\subsection{Training Losses}
To simultaneously optimize semantic alignment and reconstruction fidelity, we employ a joint objective function comprising reconstructive loss and semantic alignment loss. 

\paragraph{Supervision Signals} 
We performed training under two distinct regimes: one with time-agnostic semantic supervision, and the other with time-sensitive semantic supervision.

\textit{Time-agnostic} supervision is achieved by first generating the multi-level segmentation mask $\{K_{i,t}\}_{t=1}^T$ of the object $i$ using the Segment Anything Model (SAM) on the video frames. Each mask $K_{i,t}$ is then passed through the CLIP model to obtain its corresponding embedding $f_{i,t}$. Each pixel $(x, y)$ within the mask $K_{i,t}$ is assigned the embedding $f_{i,t}$, resulting in a region-aligned feature map. It can be written as follows:
\begin{equation}
    \mS_{\mathrm{clip}} = \sum_{i=1}^{N} \sum_{t=1}^{T} f_{i,t} \cdot \mathbb{I}_{K_{i,t}}(x, y)
\end{equation}

\textit{Time-sensitive} supervision is obtained by tracking each object $i$ across frames to get masks $\{K_{i,t}\}_{t=1}^T$, generating temporally consistent, object-specific captions $C_{i,t}$ across video frames via MLLMs, embedding them into vectors $e_{i,t} = \mathrm{Enc}(C_{i,t})$, and assigning $e_{i,t}$ to all pixels $(x,y)\in K_{i,t}$ as the dynamic semantic ground-truth over time. The resulting semantic feature map is denoted as:
\begin{equation}
    \mS_{\mathrm{dynamic}} = \sum_{i=1}^{N} \sum_{t=1}^{T} e_{i,t} \cdot \mathbb{I}_{K_{i,t}}(x, y)
\end{equation}
where $\mathbb{I}_{K{i,t}}(x,y)$ is the indicator function that is 1 if pixel $(x,y)$ belongs to mask $K_{i,t}$ and 0 otherwise, and $N$ is the total number of objects.

% the resulting region-aligned embeddings are then optionally compressed via PCA 
% for storage and visualization.

\paragraph{Semantic Alignment Loss.}
% We leverage segmentation masks $\mathrm{Seg}_t$ and dense semantic maps $\mS_t$ as supervision.

The semantic feature maps $\hat{\mS}_t$ predicted by the Semantic Head are aligned with the ground truth $\mS_{gt} \in \{{\mS_{\mathrm{clip}},\mS_{\mathrm{dynamic}}}\}$ via a combination of $\mathcal{L}_1$ regression and cosine similarity. 
To suppress background noise, we compute the alignment loss only within segmented regions by applying pixel-wise masking with segmentation masks $\{K_t\}_{t=1}^T$. Here, $K_t\in\{0,1\}^{H\times W}$ denotes the segmentation map at frame $t$, where $K_t(x,y)=1$ indicates that pixel $(x,y)$ carries semantic information (is supervised) and $K_t(x,y)=0$ otherwise.

\begin{equation}
\mathcal{L}_{\mathrm{lang}}(t) = \lambda_1 \| \hat{\mS}_t^m - \mS_t^m \|_1 + \lambda_2 (1 - cos(\hat{\mS}_t^m, \mS_t^m)).
\end{equation}
where $\hat{\mS}_t^m=\hat{\mS}_t \odot K_{t}$, $\mS_t^m=\mS_{gt} \odot K_{t}$. $\lambda_1$ and $\lambda_1$ are the loss weights, and $T$ represents the number of sequence frames.


\paragraph{Reconstruction Loss.}
RGB predictions are trained with a hybrid $\mathcal{L}_1–\mathcal{L}_2$ loss:
\begin{equation}
\mathcal{L}_{\mathrm{rgb}}(t) = \lambda_{\mathrm{img}} \| \hat{\mI}_t - \mI_t \|_1 + (1 - \lambda_{\mathrm{img}}) \| \hat{\mI}_t - \mI_t \|_2^2,
\end{equation}
where $\hat{\mI}_t \in \mathbb{R}^{3\times H \times W}$ denotes the RGB image reconstructed by the RGB Head at time $t$, $\mI_t \in \mathbb{R}^{3\times H \times W}$ denotes the ground-truth input frame and $\lambda_{\mathrm{img}}\in[0,1]$ is the loss weight balancing the two terms.


\paragraph{Joint Objective.}
To ensure that the learned features are semantically discriminative while remaining visually faithful. This joint supervision is key to building robust 4D language-aware fields. The final training loss combines both components:
\begin{equation}
\mathcal{L} = \alpha \sum_{t=1}^{T} \mathcal{L}_{\mathrm{lang}}(t) + \beta \sum_{t=1}^{T} \mathcal{L}_{\mathrm{rgb}}(t),
\end{equation}
where $t\in\{1,\ldots,T\}$ indexes the frames of a training sequence of length $T$; $\mathcal{L}_{\mathrm{lang}}(t)$ denotes the per-frame masked semantic alignment loss (defined above), $\mathcal{L}_{\mathrm{rgb}}(t)$ denotes the per-frame hybrid $\mathcal{L}_1$–$\mathcal{L}_2$ reconstruction loss, and $\alpha,\beta\ge 0$ are scalar loss weights controlling the trade-off between semantic alignment and visual fidelity.










==> src/method_mh.tex <==
\section{Methodology: 4DLangVGGT}

\input{iclr2026/figure/overview}

We introduce \textbf{4DLangVGGT}, a unified framework for building \emph{language-aware 4D fields} that maintain geometric fidelity while ensuring semantic alignment. As illustrated in Figure~\ref{fig:fig2}, the framework comprises three main components: (i) a StreamVGGT-based geometry encoder that generates spatio-temporal geometric representations (Sec.~4.1), (ii) a Semantic Bridging Decoder (SBD) that maps geometry tokens into a language-aligned semantic space (Sec.~4.2), and (iii) a multi-objective training strategy that jointly optimizes semantic alignment and appearance reconstruction (Sec.~4.3). Together, these components provide a robust foundation for 4D perception that is both structurally faithful and semantically interpretable.

\subsection{StreamVGGT-based Geometry Encoder}
As mentioned in the preliminaries and Eq. (\ref{eq:streamvggt}), the StreamVGGT aggregator alternates between \emph{spatial attention} and \emph{causal temporal attention}, producing geometry tokens $\{\mG_t\}_{t=1}^T$ that encode both fine-grained 3D geometry structure and temporal dynamics. In our framework, we adopt this architecture but keep it frozen during training. The reason is twofold: (i) StreamVGGT has already been pre-trained on large-scale video data for geometry reconstruction, providing strong spatio-temporal representations that generalize well to diverse scenes; and (ii) freezing this part avoids redundant optimization and reduces computational cost, allowing the training process to focus on semantic alignment rather than relearning geometry from scratch. 

We exclusively leverage these geometry tokens $\mG_t$ without using the camera tokens $\mC_t$. This design ensures a geometry-centered representation that forms the basis for semantic alignment. The focus of our method is not camera parameter estimation but robust semantic grounding in dynamic scenes, where geometry tokens already encode sufficient spatio-temporal information.
Formally, the process can be expressed as:
\begin{equation}
\mF_t = \mathcal{E}(\mI_t); \quad \mG_t = \mathcal{D}\left(\mF_t\ |\ \sM_{t-1}\right), \quad \text{where}\quad \sM_t = \sM_{t-1} \cup \mF_t.
\end{equation}
The StreamVGGT-based encoder provides a strong, geometry-centered foundation for our framework, enabling reliable spatio-temporal representations to support subsequent semantic alignment.


\subsection{Semantic Bridging Decoder (SBD)}
While geometry tokens capture the geometry structural and temporal dynamics of a scene, they remain agnostic to semantics and cannot directly align with natural language queries. To address this gap, we propose the Semantic Bridging Decoder (SBD), whose goal is to establish a robust mapping between geometry representations and language semantics, thereby unifying geometric fidelity and semantic alignment.

\textbf{Geometry-to-Contextual Representation Transformation.}
The input geometry tokens $\{\mG_t\}_{t=1}^T$ are first processed by a Dense Prediction Transformer (DPT)~\citep{ranftl2021vision}. As a dense prediction architecture, DPT ( $\mathcal{H}_\mathrm{DPT}$) combines the spatial sensitivity of local convolutional operations with the global modeling capability of Transformers, enabling it to capture long-range dependencies across both spatial and temporal dimensions. Through stacked self-attention layers, DPT transforms the geometry tokens into contextually enriched feature representations $\{\mH_t\}_{t=1}^T$, thereby enhancing their semantic discriminability:
\begin{equation}
\mH_t = \mathcal{H}_\mathrm{DPT}(\mG_t),\quad \forall t \in [1, \cdots, T],
\end{equation}
where $\mH_t \in \mathbb{R}^{h \times w \times c}$ is referred to as contextual tokens. Here, $h$ and $w$ denote the spatial resolution of the token map, while $c$ is the feature dimension after transformation. Importantly, this module remains trainable during optimization, allowing it to be continuously refined for semantic tasks.
    

\textbf{Dual-head Semantic and Reconstruction Decoding.} Once the contextual features $\mH_t$ are obtained, they are passed through two independent prediction heads that project them into complementary semantic and visual subspaces for dual supervision:
\begin{equation}\label{eq:dual_head}
    \hat{\mS}_t = f_{\mathrm{Lang}}(\mH_t), \quad \hat{\mI}_t = \sigma\!\left(f_{\mathrm{RGB}}(\mH_t)\right), \quad \forall t \in [1, \cdots, T],
\end{equation}
where $f_{\mathrm{Lang}}$ maps the features into a $d$-dimensional semantic embedding space for language alignment, yielding $\hat{\mS}_t \in R^{h \times w \times d}$, which serves as the predicted semantic representation at time $t$. Meanwhile, $f_{\mathrm{RGB}}$ projects the features back into the image space to reconstruct RGB frames, producing $\hat{\mI}_t \in R^{H \times W \times 3}$, which represents the reconstructed videos at time $t$ and thereby enforces perceptual consistency. Here, $H$ and $W$ denote the spatial resolution of video frames.


\subsection{Multi-objective Training}

\textbf{Semantic Loss.}
During training, we employ two complementary types of semantic supervision: time-agnostic semantic supervision and time-sensitive semantic supervision. The former provides static, object-level constraints, while the latter captures temporally evolving semantics, and together they enhance the model’s ability to achieve robust semantic alignment. For each video, we first use Segment Anything Model (SAM)~\citep{kirillov2023segment} and DEVA~\citep{cheng2023tracking} to generate its object-level masks $\{\mM_{i,t}\}_{i,t=1,1}^{N,T}$, where $i$ denotes the object index with $N$ objects in total.

\textit{Time-agnostic semantic supervision.}
Each mask region is passed through CLIP~\citep{radford2021learning} to obtain its object-specific embedding, which is then assigned to all pixels within the mask region, yielding a region-aligned semantic feature map:
\begin{equation}
\ve^{\mathrm{CLIP}}_{i,t} = f_\mathrm{CLIP}(\mI_t \cdot \mM_{i,t}), \quad\mS^{\mathrm{CLIP}}_t = \sum\nolimits_{i=1}^{N} \ve^{\mathrm{CLIP}}_{i,t} \cdot \mM_{i,t}, \quad \forall t \in [1, \cdots, T]
\end{equation}
where the CLIP embedding is denoted as $\ve^{\mathrm{CLIP}}_{i,t} \in R^{1\times 1 \times d}$, and the object mask $\mM_{i,t} \in R^{h\times w\times 1}$ takes the value 1 if a pixel belongs to the object and 0 otherwise. % $N$ is the total number of objects.

\textit{Time-sensitive semantic supervision.}
Using SAM masks across frames, we feed the video-level regions corresponding to each object into a multimodal large language model ($f_\mathrm{MLLM}$) to generate detailed and temporally consistent descriptions. These descriptions are then encoded by a large language model ($f_\mathrm{LLM}$) to obtain the corresponding semantic embeddings, which will be assigned to all pixels within the mask, producing dynamic semantic ground truth:
\begin{equation}
\{\ve^{\mathrm{dyn}}_{i,t}\}_{t=1}^T = f_\mathrm{LLM}\left(f_\mathrm{MLLM}(\{\mI_t \cdot \mM_{i,t}\}_{t=1}^T)\right), \quad \mS_t^{\mathrm{dyn}} = \sum\nolimits_{i=1}^{N} \ve^{\mathrm{dyn}}_{i,t} \cdot \mM_{i,t}.
\end{equation}

\textit{Final semantic supervision.} The semantic maps $\hat{\mS}_t$ predicted by the Semantic Head in Eq. (\ref{eq:dual_head}) are aligned with ground truth $\mS_t \in \{\mS_t^{\mathrm{CLIP}}, \mS_t^{\mathrm{dyn}}\}$ using a combination of $\mathcal{L}_1$ regression and cosine similarity.
\begin{equation}
\mathcal{L}_{\mathrm{lang}} = \sum\nolimits_{t=1}^T \lambda_1 | \hat{\mS}_t - \mS_t |_1 + \lambda_2 \left(1 - \cos(\hat{\mS}_t, \mS_t)\right), \quad \forall \mS_t \in \{\mS_t^{\mathrm{CLIP}}, \mS_t^{\mathrm{dyn}}\}.
\label{eq:lang_loss}
\end{equation}
Here, $\lambda_1$ and $\lambda_2$ are loss weights. This dual supervision scheme enables the model to learn both static object-level semantics and temporally dynamic semantics, thereby improving alignment in dynamic scenes.

\paragraph{Reconstruction Loss.}  
To ensure perceptual fidelity, the reconstructed RGB frames are supervised using a hybrid $\mathcal{L}_1$–$\mathcal{L}_2$ objective:  
\begin{equation}
\mathcal{L}_{\mathrm{rgb}} = \sum\nolimits_{t=1}^T \lambda_{\mathrm{img}} \, \| \hat{\mI}_t - \mI_t \|_1 + (1 - \lambda_{\mathrm{img}}) \, \| \hat{\mI}_t - \mI_t \|_2^2,
\label{eq:rgb_loss}
\end{equation}
where $\hat{\mI}_t$ is the frame reconstructed by the RGB Head in Eq. (\ref{eq:dual_head}), $\mI_t$ is the ground-truth input frame. $\lambda_{\mathrm{img}} \in [0,1]$ controls the trade-off between the structural accuracy ($\mathcal{L}_1$) and the pixel-level smoothness ($\mathcal{L}_2$).  

\paragraph{Final Joint Objective.}  
To jointly preserve semantic alignment and visual fidelity, we employ a dual-supervision scheme. The overall training objective is defined as
\begin{equation}
    \mathcal{L} = \alpha \mathcal{L}_{\mathrm{lang}} + \beta \mathcal{L}_{\mathrm{rgb}},
\end{equation}
where $\alpha,\beta \ge 0$ control their relative contributions.  


==> src/preliminary.tex <==
\section{Preliminaries}
\paragraph{VGGT \& StreamVGGT}

\lmh{overview process:  }  % VGGT是干啥的， StreamVGGT 蒸馏+causal+KV cache。
% y = dec(enc(x))

% 4DLangVGGT: z = SBD(y)



VGGT (Visual Geometry Grounded Transformer) is a feed-forward Transformer that, given one or many views of a scene, directly predicts key 3D attributes—including camera parameters, depth maps, point maps, and 3D point tracks—in a single pass, achieving fast and accurate reconstruction. 
Given a set of images $\{I_t\}_{t=1}^T$, where each frame $I_t \in \mathbb{R}^{3 \times H \times W},$ The processing of VGGT can be represented as:
\begin{equation}
    \mF_t = \mathcal{E}(\mI_t),\ \mG_t = \mathcal{D}(\mF_t),\ (\mP_t, \mC_t) = \mathcal{H}(\mG_t),
\end{equation}
Here, $\mathcal{E}$ represents the image encoder processing the input image $I_t$ to obtain image tokens $F_t$. $\mathcal{D}$ is a network layer that alternates between frame-level and global-level self-attention and it produces geometry tokens $G_t$. Ultimately, the predictions for both the external and internal parameters of the camera $C_t$, along with any dense outputs $P_t$, will be obtained through multiple heads $\mathcal{H}$.

StreamVGGT adapts VGGT to the streaming setting by processing incoming frames incrementally with causal temporal attention and memory of past tokens, trading some global context for real-time capability. StreamVGGT is trained with knowledge distillation from VGGT to preserve geometric fidelity while remaining efficient. Therefore, the process of obtaining the geometry token for StreamVGGT can be written as:

% \begin{equation}
% G_t = \mathcal{D}(F_t,\; \mathrm{KV}(\{F_\tau\}_{\tau=1}^{t-1})\bigr),
% \end{equation}


\begin{equation}
\mG_t = \mathcal{D}(\mF_t,\; \sM_{t-1}), \qquad \sM_t = \sM_{t-1} \cup \mathrm{KV}(\mG_t),
\end{equation}

where $\mathcal{D}$ produces the feature token $\mG_t$ by attending only to those past tokens, thereby ensuring temporal causal consistency. To avoid recomputing key–value pairs over all historical frames, \(\sM_{t}\) denotes the memory bank consisting of cached key–value pairs from past feature tokens.
This yields bounded memory and latency, enabling 4D streaming reconstruction. 

The $G_t$ obtained from StreamVGGT contains rich geometric information and is highly effective for 3D scene inference. However, its semantic grounding remains insufficient. Therefore, we propose Semantic Bridging Decoder(SBD) for semantic alignment, which can be expressed as:
\begin{equation}
    \mL_t = g_\mathrm{SBD}(\mG_t),
\end{equation}
where $\mL_t$ represents the language features of $I_t$, obtained through SBD. The specific structure of SBD is detailed in Section \ref{sec:SBD}.
% StreamVGGT introduces two key designs: 
% \begin{itemize}

% \item[(i)] \emph{Temporal causal attention} 

 
% At time step \(t\), given the current input frame \(\mI_t\) and all previous feature tokens \(\{F_\tau\}_{\tau=1}^{t-1}\), the model produces the feature token \(F_t\) by attending only to those past tokens, thereby ensuring temporal causal consistency:



% \(\mathrm{KV}(\cdot)\) denotes extraction of key–value pairs from past feature tokens, and \(f_\mathrm{Aggregator}(\cdot)\) implements a causal attention mechanism: the query is derived from \(I_t\), and the keys/values are from \(\{F_\tau\}_{\tau=1}^{t-1}\).

% \item[(ii)] \emph{Cached memory tokens} 
% To avoid recomputing over all historical frames, StreamVGGT stores the past key–value pairs in a memory bank \(M_{t-1}\), and performs incremental updates: 
% \begin{equation}
% Z_t = f_{\mathrm{Aggregator}}(F_t, M_{t-1}), \qquad
% M_t = M_{t-1} \cup \text{KV}(F_t),
% \end{equation}
% Where \(Z_t\) denotes the aggregated representation at time \(t\), and \(M_t\) is the updated memory bank. 

% To avoid recomputing key–value pairs over all historical frames, we maintain a memory bank \(M_{t-1}\) consisting of cached key–value pairs from past feature tokens. When a new feature token \(F_t\) is computed at time step \(t\), we extract its key–value pair \(\mathrm{KV}(F_t)\) and update the memory:

% \begin{equation}
% \sM_t = \sM_{t-1} \cup \mathrm{KV}(F_t),
% \end{equation}
% where \(M_t\) is the memory bank after time \(t\).  During inference, queries at timestep \(t'\) attend only to key–value entries in the memory bank \(\sM_{t'-1}\), reducing computation and avoiding redundant recomputation over past frames.

% \end{itemize}



% \paragraph{4D Reconstructive Tokenization}
% In our framework, we reinterpret the aggregation process of StreamVGGT as a \emph{4D reconstructive tokenization} step. Instead of explicitly producing point clouds or meshes, StreamVGGT maps each incoming monocular frame $\mI_t$ into latent tokens:


% \begin{equation}
% \mR_t = \phi_{\mathrm{enc}}(\mI_t) \in \sR^{M \times d}, \qquad \mR_t = \{\mR_t^{\text{feat}},\; \mR_t^{\text{view}}\}.
% \end{equation}


% where $\mR_t^{\mathrm{}{feat}}$ denotes the feature tokens used to encode local scene geometry and $\mR_t^{\text{view}}$ denotes the camera-view tokens to encode perspective information.

% The joint set $mR_t$ constitutes a compact \emph{4D reconstructive token} representation, implicitly capturing observed 3D geometry and camera poses across time. Unlike explicit 3D structures (e.g., voxels or point clouds), $\mR_t$ provides a continuous, latent, and temporally causal encoding suitable for downstream 4D reasoning and reconstruction tasks.


==> src/statement.tex <==
\paragraph{Ethics Statement.}
We follow the ICLR Code of Ethics. Our work focuses on building 4D language fields for dynamic scene understanding and does not involve personal data, sensitive attributes, or identifiable human subjects beyond synthetic or publicly available datasets. Specifically, we conduct experiments on HyperNeRF and Neu3D, which are license-compliant research datasets containing synthetic or anonymized real-world scenes. We exclude any content that is violent, sexual, or otherwise harmful. The semantic annotations used in our work are automatically generated through established vision–language models (e.g., CLIP, SAM, DEVA) and do not involve manual collection of biometric or medical data. While our method learns semantic representations for 4D dynamic scenes, it does not involve identity-related, biometric, or personally sensitive data. The semantic features are derived from publicly available datasets and pretrained vision–language models, and do not enable identity reconstruction or manipulation. The release is restricted to research purposes only, with terms prohibiting harmful or deceptive uses. This study complies with all applicable policies on privacy, copyright, and research integrity.

\paragraph{Reproducibility Statement.}
We ensure reproducibility by providing a complete description of the 4DLangVGGT framework, including detailed formulations of the StreamVGGT-based geometry encoder, the Semantic Bridging Decoder, and the multi-objective training objective. Hyperparameters, loss weights, and dataset splits are clearly specified in the main text and appendix. We will release code, pretrained models to reproduce all reported results. Our supplementary materials include qualitative video visualizations on HyperNeRF and Neu3D. Together, these materials ensure that all results in the paper can be independently verified and extended.

==> tab/tab1.tex <==
\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{3pt}
    \caption{Quantitative comparison of \textbf{time-agnostic querying} on the HyperNeRF dataset} 
    \label{tab:time_sensitive_hypernerf}
    \vspace{-2mm}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccccccccc}
        \toprule
        \multirow{2}{*}{\centering Method} & \multicolumn{2}{c}{\textbf{americano}} & \multicolumn{2}{c}{\textbf{chick-chicken}} & \multicolumn{2}{c}{\textbf{split-cookie}} & \multicolumn{2}{c}{\textbf{torchocolate}} & \multicolumn{2}{c}{\textbf{Average}}\\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
        & \textbf{mIoU(\%)} & \textbf{mAcc(\%)} & \textbf{mIoU(\%)} & \textbf{mAcc(\%)} & \textbf{mIoU(\%)} & \textbf{mAcc(\%)} & \textbf{mIoU(\%)} & \textbf{mAcc(\%)} & \textbf{mIoU(\%)} & \textbf{mAcc(\%)}\\
        \midrule
        LangSplat~\citep{qin2024langsplat} & 72.08 & 97.61 & 75.98 & 97.86 & 76.54 & 97.32 & 69.55 & 98.09 &73.54 &97.72 \\
        Feature-3DGS~\citep{zhou2024feature} & 34.65 & 62.96 & 47.21 & 87.22 & 47.03 & 68.25 & 24.71 & 64.58 &38.40 &70.75\\
        Gaussian Grouping~\citep{ye2024gaussian} & 61.77 & 71.31 & 34.65 & 75.52 & 72.71 & 96.56 & 58.95 & 85.52 &57.02 &82.22\\
        4DLangSplat~\citep{li20254d} & 83.48 & \underline{98.77} & 86.50 & 98.81 & 90.04 & 98.67 & 71.79 & 98.10 &82.95 &98.59\\
        \midrule
        4DLangVGGT (Ours \& per-scene) & \textbf{86.45} & \textbf{98.95} & \textbf{90.70} & \textbf{99.03} & \underline{90.15} & \underline{98.79} & \underline{72.77} & \underline{98.32} &\textbf{85.02} &\textbf{98.77} \\ %%% Add general result
        4DLangVGGT (Ours) & \underline{82.46} & 98.36 & \underline{86.91} & \underline{98.88} & \textbf{91.44} & \textbf{98.87} & \textbf{75.15} & \textbf{98.57} &\underline{83.99} &\underline{98.67} \\
        \bottomrule
    \end{tabular}
}
\end{table}

==> tab/tab2.tex <==
\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{3pt}
    \caption{Quantitative comparison of \textbf{time-sensitive querying} on the HyperNeRF dataset} 
    \label{tab:time_sensitive_hypernerf}
    \vspace{-2mm}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccccccccc}
        \toprule
        \multirow{2}{*}{\centering Method} & \multicolumn{2}{c}{\textbf{americano}} & \multicolumn{2}{c}{\textbf{chick-chicken}} & \multicolumn{2}{c}{\textbf{split-cookie}} & \multicolumn{2}{c}{\textbf{espresso}} & \multicolumn{2}{c}{\textbf{Average}} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
        & \textbf{Acc(\%)} & \textbf{vIoU(\%)} & \textbf{Acc(\%)} & \textbf{vIoU(\%)} & \textbf{Acc(\%)} & \textbf{vIoU(\%)} & \textbf{Acc(\%)} & \textbf{vIoU(\%)} & \textbf{Acc(\%)} & \textbf{vIoU(\%)} \\
        \midrule
        LangSplat~\citep{qin2024langsplat} & 45.19 & 23.16 & 53.26 & 18.20 & 73.58 & 33.08 & 44.03 & 16.15 & 54.01 & 22.65 \\
        Deformable CLIP & 60.57 & 39.96 & 52.17 & 42.77 & 89.62 & 75.28 & 44.85 & 20.86 & 61.80 & 44.72 \\
        Non-Status Field & 83.65 & 59.59 & 94.56 & 86.28 & 91.50 & 78.46 & 78.60 & 47.95 & 87.58 & 68.57 \\
        4DLangSplat~\citep{li20254d} & 89.42 & 66.07 & 96.73 & 90.62 & 95.28 & 83.14 & 81.89 & 49.20 & 90.83 & 72.26 \\
        \midrule
        4DLangVGGT (Ours \& per-scene) & 89.96 & 66.78 & 98.01 & 93.56 & 95.56 & 83.44 & 82.44 & 51.56 & 90.86 & 73.06 \\
        4DLangVGGT (Ours)  & 90.03 & 67.77 & 97.81 & 93.44 & 95.76 & 84.02 & 82.86 & 52.06 & 91.44 & 74.74 \\
        \bottomrule
    \end{tabular}
}
\end{table}
